HiDeNN-PGD: reduced-order hierarchical deep learning neural networks

This paper presents a proper generalized decomposition (PGD) based reduced-order model of hierarchical deep-learning neural networks (HiDeNN). The proposed HiDeNN-PGD method keeps both advantages of HiDeNN and PGD methods. The automatic mesh adaptivity makes the HiDeNN-PGD more accurate than the finite element method (FEM) and conventional PGD, using a fraction of the FEM degrees of freedom. The accuracy and convergence of the method have been studied theoretically and numerically, with a comparison to different methods, including FEM, PGD, HiDeNN and Deep Neural Networks. In addition, we theoretically showed that the PGD converges to FEM at increasing modes, and the PGD error is a direct sum of the FEM error and the mode reduction error. The proposed HiDeNN-PGD performs high accuracy with orders of magnitude fewer degrees of freedom, which shows a high potential to achieve fast computations with a high level of accuracy for large-size engineering problems.

==> Part1_Oldversion.tex <==
\section{ DNN, HiDeNN, FEM and canonical decomposition based function approximation}

Function approximation is a key component in numerical solutions of partial differential equations (PDEs). In this section, we briefly review how such approximation can be performed in terms of FEM, DNN, HiDeNN and canonical decomposition (CD). We present their approximation function sets, which will be used in the theoretical analysis in Subsection 2.2.
We restrict the discussion to a scalar-value function ${u}(\bm{x}):\mathbb{R}^3\rightarrow \mathbb{R}$. The conclusions should be straightforwardly extended to vector functions.

\begin{figure}[h]
	\centering
	\subfigure[DNN-based interpolation function]{\includegraphics[trim={1.2cm 0 0 0},width=0.41\textwidth]{NNShapeDNN.png}}
	\subfigure[HiDeNN interpolation function]{\includegraphics[width=0.45\textwidth]{HiDeNN_DNN.png}}
	\subfigure[FEM interpolation function]{\includegraphics[width=0.45\textwidth]{FEM_DNN.png}}
	\subfigure[CD interpolation function]{\includegraphics[width=0.45\textwidth]{MS_DNN.png}}
	\caption{Illustration for the interpolation functions in the form of DNN with $\bm{x}=(x,y,z)$ as input and $u^h$ as output. Weights and biases inside dashed line-box are constrained, and those inside the red solid line-box are fixed. }
	\label{fig:Interpolant_DNNrepresentation}
\end{figure}

\subsection{Overview of the approximation function sets}
\textbf{Deep Neural network based method}

According to the universal approximation theorem, a deep neural network (DNN) can be designed and trained to approximate any given continuous function to desired accuracy \cite{hornik1989multilayer,cybenko1989approximation}. Thus it can be a candidate to  approximate solutions for solving PDEs \cite{wu2016physics,xiao2016quantifying,weinan2017deep,berg2018unified,raissi2017physics,raissi2019physics,sirignano2018dgm,weinan2018deep}, i.e.
\begin{equation}
    u^h(\bm{x})=\mathcal{F}^{NN}(\bm{x})
\end{equation}
where $\mathcal{F}^{NN}$ represents the neural network with $\bm{x}$ as input and $u^h$ as output. Note that $u^h$ can be a multidimensional vector.
For instance, in a classical feedforward neural network (FFNN) \cite{Goodfellow-et-al-2016,haykin1994neural,oishi2017computational} with $N_L$ layers, recursive relations among neurons are as follows
%Weinan E and bing Yu \cite{} proposed the Deep Ritz Method by using the neural network representation of functions to solve variational problems.
% \begin{eqnarray} \label{eq:transfer-function}
% a^{l}_j &=&
% \begin{cases}
% x_j, \text{ if } l=1 \text{ (input layer)} \\
% \mathscr{A}(\sum_{i=1}^{N_N(l-1)}{W^{l}_{ij} a^{l-1}_i + b^{l}_j}), \text{ if } l\in\{2,...,N_L-1\}  \text{ (hidden layer)}
% \end{cases}
% \end{eqnarray}
\begin{eqnarray} \label{eq:transfer-function}
&&a^{l}_{j=1}=x, a^{l}_{j=2}=y, a^{l}_{j=3}=z, \text{ if } l=1 \text{ (input layer)} \\
&&a^{l}_j=\mathscr{A}(\sum_{i=1}^{N_N(l-1)}{W^{l}_{ij} a^{l-1}_i + b^{l}_j}), \text{ if } l\in\{2,...,N_L-1\}  \text{ (hidden layer)}
\end{eqnarray}
Hence, the output layer can be defined as
\begin{eqnarray}
\mathcal{F}^{NN}_j&=&a^{N_L}_j=\sum_{i=1}^{N_N(N_L-1)}{W^{N_L}_{ij} a^{N_L-1}_i + b^{N_L}_j}, \text{ if } l=N_L \text{ (output layer)}
\end{eqnarray}
%where $N_L$ denotes the number of layers, $a_j^l$ the neuron value for $j$th neuron in $l$th layer,  $W^l_{i,j}$ the weight connecting the $i$th neuron in layer $l-1$ to the $j$th in layer $l$, $b^l_j$ denotes the bias of the $j$th neuron in layer $l$ and $\mathcal{A}$ the activation function.
with the detailed definition of the notations in Table \ref{table:ffnn-notation}. Therefore, once the weights $\bm{W}$, biases $\bm{b}$ and activation functions $\bm{\mathcal{A}}$ have been chosen, $\mathcal{F}^{NN}$ can serve as an approximation function with the input variable as $\bm{x}=(x,y,z)$. 

\begin{table}[h!]
\centering
\caption{Notation table of variables used in the feed forward neural network} 
\label{table:ffnn-notation}
\begin{tabular}{cl}
  \hline
      $\bm{x}=(x,y,z)$ & Space coordinates \\
      $l$ & Counting index for number of layers \\
      $i$ & Counting index for neurons in layer $l-1$ \\
      $j$ & Counting index for neurons in layer $l$ \\
      $N_L$ & Number of layers in the neural network \\
      $N_N(l)$ & Number of neurons in layer $l$ \\
      $W_{ij}^{l}$ & Weight connecting the $i^\text{th}$ neuron in layer $l-1$ to the $j^\text{th}$ in layer $l$ \\
      $b_{j}^{l}$ & Bias of the $j^\text{th}$ neuron in layer $l$\\
      $a_j^{l}$ & Neuron value for $j^{th}$ neuron in $l^{th}$ layer \\
      $\mathscr{A}$ & Activation function \\
      $\mathcal{F}^{NN}$ & Feedforward neural network function\\
 \hline
\end{tabular}
\end{table}

The approximation function set formed by a general NN is
\begin{equation}
    \mathcal{N}^h=\left\{ u^h(\bm{x}) \big | u^h=\mathcal{F}^{NN}(\bm{x};\bm{W},\bm{b},\bm{\mathscr{A}}), W^l_{ij}\in \mathbb{R}, b^l_j\in \mathbb{R} \right\},
\end{equation}
where $\mathcal{F}^{NN}(\bm{x};\bm{W},\bm{b},\bm{\mathcal{A}})$ denotes an NN with the input $\bm{x}$ and depends on weights $\bm{W}$, biases $\bm{b}$ and activation functions $\bm{\mathcal{A}}$.

For interpretation, NN can be somehow  written in the form of shape functions associated to nodal values of $ u^h$. This way, the function approximation reads
\begin{equation}
    u^h=\sum_{I=1}^{np} \mathcal{F}^{NN}_\mathcal{I}(\bm{x};\bm{W},\bm{b},\bm{\mathscr{A}}) \mathscr{u}_{\mathcal{I}},
    \label{eq:InterpolationNN}
\end{equation}
As illustrated in Fig. \ref{fig:Interpolant_DNNrepresentation}(a), the equation \eqref{eq:InterpolationNN} would define a specific structure of DNN. The blue blocks in the figure denoted by $\mathcal{F}^{NN}_{\mathcal{I}}(\bm{x};\bm{W},\bm{b},\bm{\mathscr{A}})$ is a DNN substructure with $\bm{x}$ as input and $\mathcal{F}^{NN}_{\mathcal{I}}$ as output, which has a similar definition to \eqref{eq:transfer-function}. $u_I$'s are actually the weights connecting the output layer with the last hidden layer.
%Examples of constraints for such shape functions can be
% \begin{eqnarray}
%     \sum_{I=1}^{np} \mathcal{F}^{NN}_I(\bm{x};\bm{W},\bm{b},\bm{\mathcal{A}})=1, \mathcal{F}^{NN}_I(\bm{x}_J;\bm{W},\bm{b},\bm{\mathcal{A}})=\delta_{IJ},
%     \label{eq:Constraint}
% \end{eqnarray}
% with $\delta_{IJ}$ denoting the Kronecker delta. The corresponding nodal values denoted by $u_I$ are introduced as weights in the last layer.
Compared to DNN, this interpolation form may provide a more interpretable structure for the weights and biases. 

In multidimensional cases, such as for 3D mechanical problems, the above equation can be straightforwardly applied to each component of displacement fied as follows
\begin{equation}
    u_x^h=\sum_{I=1}^{np} \mathcal{F}^{NN}_\mathcal{I}(\bm{x};\bm{W},\bm{b},\bm{\mathscr{A}}) \mathscr{u}_x_{\mathcal{I}},\\
\end{equation}
\begin{equation}
    u_y^h=\sum_{I=1}^{np} \mathcal{F}^{NN}_\mathcal{I}(\bm{x};\bm{W},\bm{b},\bm{\mathscr{A}}) \mathscr{u}_y_{\mathcal{I}},
\end{equation}
\begin{equation}
    u_z^h=\sum_{I=1}^{np} \mathcal{F}^{NN}_\mathcal{I}(\bm{x};\bm{W},\bm{b},\bm{\mathscr{A}}) \mathscr{u}_z_{\mathcal{I}},
\end{equation}

% In this work, we restrict our theoretical discussion to the single component case, but the conclusion should hold for multidimensional cases.

%If we require constraints for  $\mathcal{F}^{NN}_I(\bm{x};\bm{W},\bm{b},\bm{\mathcal{A}})$, this form might be more efficient with constrained DoFs. The key point of this form of approximation is to find an efficient way to construct $\mathcal{F}^{NN}_I(\bm{x};\bm{W},\bm{b},\bm{\mathcal{A}})$ under desired constraints \eqref{eq:Constraint}.
%The NN based approaches then search the solution in the set $\mathcal{N}^h$ by minimizing the loss function, which is related to the energy potential $\Pi[u]$ in our case.

% \begin{figure}[h]
% 	\centering
% 	\includegraphics[width=0.9\textwidth]{NeuralNetwork.png}
% 	\caption{Illustration of a classical feedforward neural network (FFNN). A general FFNN contains neurons (the circles) and weights (black lines). An FFNN consists of one input layer (green), one output layer (orange), and multiple hidden layers (blue). As an interpolation function, the input is space coordinates $\bm{x}=(x,y,z)$. $\mathcal{F}^{NN}$ denotes the output. $N_L$ denotes the number of layers. $a_j^l$ denotes the neuron value for $j$th neuron in $l$th layer.  $W^l_{i,j}$ denotes the weight connecting the $i$th neuron in layer $l-1$ to the $j$th in layer $l$. $b^l_j$ denotes the bias of the $j$th neuron in layer $l$. $\mathcal{A}$ denotes the activation function. The formula to connect neurons of two adjacent layers is $a_j^l=\mathcal{A}(\sum_i W^l_{i,j} a_i^{l-1} +b_j^l)$.}
% 	\label{fig:NeuralNetwork}
% \end{figure}

\textbf{HiDeNN}

 %Recently, we combined the FEM and NN and proposed a systematic way to construct a class of structured deep neural networks for solving PDEs \cite{zhang2020hierarchical}.
 The recently developed HiDeNN method \cite{zhang2020hierarchical} uses a similar DNN structure of \eqref{eq:InterpolationNN} with additional constraints to build a family of function approximations. Similarly to the  FEM, the continuous domain
$\Omega$ is discretized by a mesh with $np$ nodes $\bm{x}_1,\bm{x}_2,\cdots,\bm{x}_{np}$. Then the finite element shape functions $N_{\mathcal{I}}$ can be constructed by the neural network block, namely, 
\begin{equation}
     \mathcal{N}_{\mathcal{I}}(\bm{x};\bm{W},\bm{b},\bm{\mathscr{A}})
\end{equation}
where $\mathcal{I}=1,2,\cdots,np$. Different from $\mathcal{F}_{\mathcal{I}}^{NN}(\bm{x};\bm{W},\bm{b},\bm{\mathcal{A}})$ in (\ref{eq:InterpolationNN}), $\mathcal{N}_{\mathcal{I}}(\bm{x};\bm{W},\bm{b},\bm{\mathcal{A}})$ precisely equals to the finite element shape function $N_{\mathcal{I}}(\bm{x})$ with inputs $\bm{x}$ and an output $N_{\mathcal{I}}$, satisfying the following constraints for  shape functions automatically, i.e.
\begin{eqnarray}
    \sum_{\mathcal{I}=1}^{np} \mathcal{N}_{\mathcal{I}}(\bm{x};\bm{W},\bm{b},\bm{\mathscr{A}})=1, \mathcal{N}_{\mathcal{I}}(\bm{x}_{\mathcal{J}};\bm{W},\bm{b},\bm{\mathscr{A}})=\delta_{\mathcal{I}\mathcal{J}}.
    \label{eq:Constraint}
\end{eqnarray}
With Kronecker Delta constraints, we can apply Dirichlet boundary conditions directly similar to that of the finite element method, 
so that all the weights $\bm{W}$,  and biases $\bm{b}$ are functions of nodal coordinates $\bm{x}_I$. Thus we can rewrite the shape function explicitly in terms of $\bm{x}_I$ as
\begin{equation}
    \mathcal{N}_{\mathcal{I}}(\bm{x};\bm{x}_{\mathcal{I}}^*,\bm{\mathscr{A}}) = \mathcal{N}_{\mathcal{I}}(\bm{x};\bm{W},\bm{b},\bm{\mathscr{A}}),
\end{equation}
where $\bm{x}_{\mathcal{I}}^*$ denotes the support of $N_{\mathcal{I}}(\bm{x})$, e.g. in linear 1D cases $\bm{x}_{\mathcal{I}}^*=[x_{{\mathcal{I}}-1},x_{\mathcal{I}},x_{{\mathcal{I}}+1}]$.

Combining such neural network blocks for the entire mesh gives the final form of HiDeNN, as shown in Fig. \ref{fig:1D_DNN_representation}(b). This results in the approximation function set
\begin{equation}
    \mathcal{H}^h=\left\{ u^h(\bm{x}) \bigg | u^h=\sum_{\mathcal{I}=1}^{np} \mathcal{N}_{\mathcal{I}}(\bm{x};\bm{x}_{\mathcal{I}}^*,\bm{\mathcal{A}})\mathscr{u}_{\mathcal{I}}, \mathscr{u}_{\mathcal{I}}\in\mathbb{R} \right\}.
\end{equation}
% \begin{equation}
%     \mathcal{HI}^h=\left\{ u^h \bigg | u^h=\sum_{I=1}^{np} \mathcal{N}_I(\bm{x};\bm{x}_I^*,\bm{\mathcal{A}})\mathscr{u}_I, \mathscr{u}_I\in\mathbb{R}, \text{ and } \mathscr{u}_I=0, \forall x_I\in\partial\Omega \right\}.
% \end{equation}
% As illustrated in Fig. \ref{fig:Interpolant_DNNrepresentation}(b), the corresponding DNN consist of two parts: shape functions represented by DNN and nodal values introduced as weights in the last layer. 
% It can be noticed that the interpolant is determined by nodal positions, activation functions and nodal values. Hence, the optimization process in HiDeNN concerns finding the optimal supporting mesh and the nodal values. 
% %which reads 
% % \begin{equation}
% %     \bm{u}^h=\argmin_{\bm{u}^{h*} \in \mathcal{HI}^h, \bm{x}_I^*\in \Omega} \Pi[\bm{u^{h*} }]
% % \end{equation}
% It has been shown that optimizing the mesh results in an automatic r-adaptivity which improves the local and global accuracy of the interpolant. By fixing the depth of the
% hidden layers, rh-adaptivity can be achieved by adding neurons for higher accuracy within the optimization process. 

The parametric expression with nodal positions $\bm{x}_{\mathcal{I}}^*$ allows automatic r-adaptivity, and accordingly improves the local and global accuracy of the interpolant.

\textbf{Finite element method}

The approximation function set $\mathcal{HI}^h$ degenerates to the FE approximation function set $\mathcal{V}^h$ \cite{belytschko2013nonlinear} when the nodal position is fixed, which reads
\begin{equation}
    \mathcal{V}^h=\left\{u^h(\bm{x}) \bigg | u^h=\sum_{\mathcal{I}=1}^{np} N_{\mathcal{I}}(\bm{x}) u_{\mathcal{I}}, u_{\mathcal{I}}\in\mathbb{R} \right\}.
\end{equation}

From the DNN viewpoint, this corresponds to fixing the weights and biases that are functions of $\bm{x}_{\mathcal{I}}^*$, as shown in Fig. \ref{fig:Interpolant_DNNrepresentation}(b). %are fixed and determined by a given mesh.
% \begin{equation}
%     \mathcal{V}^h=\left\{u^h(\bm{x}) \bigg | u^h(\bm{x})=\sum_{I=1}^{np} N_I(\bm{x}) u_I, u_I\in\mathbb{R}, \text{ and } u_I=0, \forall x_I\in\partial\Omega \right\}.
% \end{equation}
%where  $N_I(x_J)=\delta_{IJ}$ with $\delta_{IJ}$ denoting the Kronecker delta. %The FEM solution to the problem \eqref{eq:GeneralPDE} is found by solving 
% \begin{equation}
%     \bm{u}^h=\argmin_{\bm{u}^{h*} \in \mathcal{V}^h} \Pi[\bm{u^{h*} }]
% \end{equation}

% The classical shape functions are given by virtue of parametric coordinates which maps the given element of the mesh into the unit square or cubic, as shown in Fig. \ref{}. The parametric coordinates $\bm{\xi}$ in the unit square or cubic
% are to be related to the physical coordinates $\bm{x}$
% by mapping of the form
% \begin{equation}
%     \bm{x}=\sum_{a=1}^{n_{en}} N_a^e(\bm{\xi}) \bm{x}^e_a,
% \end{equation}
% where $n_{en}$ is the number of element nodes, such as $n_{en}=4$ for 4-node element as shown in Fig. \ref{}, and $\bm{x}^e_a$ is the physical coordinates of the $a$-th node in the element. This way proposes a general way to obtain shape functions for an arbitrary mesh.


\textbf{Canonical decomposition (CD)}

Under the assumption of separation of variables, the function $\bm{u}$ may be approximated
by the sum of the products of multiple 1D functions, i.e.,
\begin{equation}
    u^h(\bm{x})=u^h(x,y,z)=\sum_{q=1}^Q X^{(q)}(x)Y^{(q)}(y)Z^{(q)}(z)
    \label{eq:SeparaRepresentation}
\end{equation}
where $Q$ is the number of modes, and the product of $X^{(q)}, Y^{(q)},Z^{(q)}$ provides a mode for the interpolation function.
This form or concept is known as canonical decomposition (CD) \cite{kolda2009tensor}. The so-called PGD method has adopted this concept for solving PDEs \cite{ammar2006new,gonzalez2010recent,ghnatios2019advanced,modesto2015proper,chinesta2013proper} and for data learning \cite{lu2018adaptive,lu2019datadriven,blal2019non, ghnatiosspurious,giacomini2020separated}. %In a general sense, the decomposition can be obtained in different ways. In our work, we adopt the terminology modal superposition (MS) for deriving our mathematical proofs.

Thanks to the separation of variables, only shape functions of reduced dimension are needed. In (\ref{eq:SeparaRepresentation}),
1D FE shape functions can be used for a 3D problem, namely,
\begin{eqnarray}
    \label{eq:MSDisX}
    X^{(q)}(x)&=&\sum_{I=1}^{n_1} N_I(x)\beta_I^{(q)}, \\
    \label{eq:MSDisY}
    Y^{(q)}(y)&=&\sum_{J=1}^{n_2} N_J(y)\gamma_J^{(q)}, \\
    \label{eq:MSDisZ}
    Z^{(q)}(z)&=&\sum_{K=1}^{n_3} N_K(z)\theta_K^{(q)}.
\end{eqnarray}
Here, $n_1, n_2, n_3$ are the number of nodes in $x,y,z$ directions, respectively.
Thus the corresponding approximation function set for a given $Q$ modes is
\begin{eqnarray}
    \mathcal{M}_Q^h=&\Bigg \{ &u^h(\bm{x}) \bigg |u^h=\sum_{q=1}^Q \left( \sum_{I=1}^{n_1} N_I(x)\beta_I^{(q)} \right) \left( \sum_{J=1}^{n_2} N_J(y)\gamma_J^{(q)} \right) \left( \sum_{K=1}^{n_3} N_K(z)\theta_K^{(q)} \right), \\ \nonumber 
    &&\beta_I^{(q)},\gamma_J^{(q)},\theta_K^{(q)}\in\mathbb{R} \Bigg \}.
\end{eqnarray}
% \begin{eqnarray}
%     \mathcal{M}_Q^h=&\Bigg \{ &u^h \bigg |u^h=\sum_{q=1}^Q \left( \sum_{i=1}^{n_1} N_i(x)\beta_i^{(q)} \right) \left( \sum_{j=1}^{n_2} N_j(y)\gamma_j^{(q)} \right) \left( \sum_{k=1}^{n_3} N_k(z)\theta_k^{(q)} \right), \\ \nonumber 
%     &&\beta_1^{(q)}=\beta_{n_1}^{(q)}=\gamma_1^{(q)}=\gamma_{n_2}^{(q)}=\theta_1^{(q)}=\theta_{n_3}^{(q)}=0, \beta_i^{(q)},\gamma_j^{(q)},\theta_k^{(q)}\in\mathbb{R},\\ \nonumber
%     &&i=2,3,\cdots,n_1-1, j=2,3,\cdots,n_2-1, k=2,3,\cdots,n_3-1 \Bigg \}.
% \end{eqnarray}

Note that the interpolation function in (\ref{eq:SeparaRepresentation}) can be rearranged as
\begin{equation}
    u^h(x,y,z)=\sum_{I=1}^{n_1}\sum_{J=1}^{n_2}\sum_{K=1}^{n_3} N_I(x) N_J(y) N_K(z) \left( \sum_{q=1}^Q \beta^{(q)}_I \gamma^{(q)}_J \theta^{(q)}_K \right)
    \label{eq:MSExpand}
\end{equation}
which is regarded as a finite element interpolation function with $N_I(x)N_J(y)N_K(z)$ as shape
functions and $\left( \sum_{q=1}^Q \beta^{(q)}_I \gamma^{(q)}_J \theta^{(q)}_K \right)$ as coefficients. Fig. \ref{fig:Interpolant_DNNrepresentation}(d) illustrates a DNN format of (\ref{eq:MSExpand}), which will be the basis for the proposed HiDeNN-PGD method.

Multidimensional shape functions of CD, i.e., the product of 1D shape functions, are fixed and determined by nodal positions along each direction. In addition, the nodal values in the last layer are constraint in the form of tensor product, i.e.,
\begin{equation}
    u_{(I,J,K)}=\sum_{q=1}^{Q}\beta^{(q)}_{I}\gamma^{(q)}_J\theta^{(q)}_K.
\end{equation}

When a few modes may represent the function $u^h(x,y,z)$, this method is advantageous in terms of lower integration complexity and less degrees of freedom (DoFs) \cite{ammar2006new,chinesta2013proper}. The DoFs in (\ref{eq:MSExpand}) is of the order $O((n_1+n_2+n_3)Q)$, which is linear with the spatial dimension and far smaller than traditional methods (e.g., FEM). 

%Classical PGD uses the same representation, and solves the problem in an incremental way \cite{ammar2006new,chinesta2013proper}. We shall give the detailed solution scheme in Section 4.
% Classical PGD uses the same representation, and solves the problem in an incremental way \cite{ammar2006new,chinesta2013proper}. More precisely, the solution scheme is
% \begin{equation}
% \begin{array}{lll}
% \text{The first mode:} &u^{PGD,(1)}=\arg \min_{\Delta u \in \mathcal{M}^h_{Q=1}} \Pi[0+\Delta u];\\
% \text{For $m>1$, the $m$-th mode:} &\Delta u^{(m)}=\arg \min_{\Delta u \in \mathcal{M}^h_{Q=1}} \Pi[u^{PGD,(m-1)}+\Delta u], \\
% \text{The PGD solution with $m$ modes:} &u^{PGD,(m)}=u^{PGD,(m-1)}+\Delta u^{(m)},
% \end{array}
% \end{equation}
% \begin{equation}
% \begin{array}{ccc}
% &&\text{The first mode:} u^{PGD,(1)}=\arg \min_{\Delta u \in \mathcal{M}^h_{Q=1}} \Pi[0+\Delta u];\\
% &&\text{For $m>1$, the $m$-th mode:} \Delta u^{(m)}=\arg \min_{\Delta u \in \mathcal{M}^h_{Q=1}} \Pi[u^{PGD,(m-1)}+\Delta u]; \\ \nonumber
% &&u^{PGD,(m)}=u^{PGD,(m-1)}+\Delta u^{(m)},
% \end{array}
% \end{equation}
%We remarked it is also possible to solve several modes simultaneously in one incremental step \cite{}.

\subsection{Relationship among the NN, HiDeNN, FEM and CD approximation function sets}

In this subsection, we explore the relationship among FEM, NN, HiDeNN and CD. 

Assume that CD, FEM are based on the same regular mesh with $n_1,n_2,n_3$ nodes along $x,y,z$ directions. This mesh also serves as an initial guess of $\bm{x}_I^*$ in HiDeNN. The shape functions of FEM is the product of 1D shape functions, i.e., the shape function associated with the node $(x_i,y_j,z_k)$ is $N_{(I,J,K)}(x,y,z)=N_I(x) N_J(y) N_K(z)$. NN has the same neural network with HiDeNN, and might be fully-connected. By definition, we have the following relationship among approximation function sets of the four methods:
\begin{equation}
    \mathcal{M}_Q^h \subset \mathcal{V}^h \subset \mathcal{HI}^h \subset \mathcal{N}^h,
    \label{eq:RelationshipAmongMethods}
\end{equation}
as illustrated in Fig. \ref{fig:Relationship}.

\begin{figure}[h]
	\centering
	\includegraphics[width=0.8\textwidth]{RelationshipFiveMethods.png}
	\caption{Illustration for relationship among interpolation function sets of CD, FEM, HiDeNN-PGD, HiDeNN and NN. Especially, when $Q$ tends to infinity, the ``distance" $\varepsilon_Q$ between $\mathcal{M}_Q^h$ and $\mathcal{V}^h$ vanishes. When $Q$ is big enough, FEM interpolation set $\mathcal{V}^h$ is the subset of HiDeNN-PGD one $\mathcal{G}^h_Q$.}
	\label{fig:Relationship}
\end{figure}

Based on the assumptions and definitions of interpolation sets of four methods, we have the following observations:
\begin{description}
	\item[$\bullet$] According to (\ref{eq:MSExpand}), the CD interpolation functions can be regarded as finite element interpolation functions, which belong to $\mathcal{V}^h$, so $\mathcal{M}_Q^h \subset \mathcal{V}^h$. Especially, when $Q$ tends to infinity, the ``distance" between these two sets vanish. Detailed results will be shown in Section 4. Proofs can be found in Appendix \ref{Appdix:2DConverge}.
	\item[$\bullet$] In HiDeNN, an optimization of the nodal positions is performed. Thus FEM may be regarded as a specific case in the HiDeNN with nodal coordinates fixed .
	\item[$\bullet$] HiDeNN is a class of structured NN with weights and biases as functions of nodal values and nodal positions.
\end{description}

% In summary, we conclude (\ref{eq:RelationshipAmongMethods}) among the four interpolation function sets. See Fig. \ref{fig:Relationship} for illustration. HiDeNN-PGD is our proposed method and will be introduced in Section \ref{sec:HiDeNNPGD}.

% \section{Interpolation theory from a point of DNN-based view}


% In this section, all interpolation functions are rewritten in a DNN format to show the difference among them from a point of DNN-based view. Fig. \ref{fig:Interpolant_DNNrepresentation} addresses the DNNs corresponding to HiDeNN, FEM, NN and MS. Similar with HiDeNN’s construction, these DNN structures consist of two parts: shape functions represented by DNN and nodal values introduced in the last layer. For consistency, NN uses the same structure but no concepts of shape functions and nodal values. We also present corresponding optimization formulas of these methods in a DNN way with the loss function denoted as $Loss(u^h)$.

% \begin{figure}[h]
% 	\centering
% 	\subfigure[HiDeNN interpolation function]{\includegraphics[width=0.45\textwidth]{HiDeNN_DNN.png}}
% 	\subfigure[FEM interpolation function]{\includegraphics[width=0.45\textwidth]{FEM_DNN.png}}
% 	\subfigure[NN-based interpolation function]{\includegraphics[width=0.45\textwidth]{NN_DNN.png}}
% 	\subfigure[MS interpolation function]{\includegraphics[width=0.5\textwidth]{MS_DNN.png}}
% 	\caption{Illustration for the interpolation functions in the form of DNN. Weights and biases in the part surrounded by dashed line are constraint, and those in the part surrounded by red solid line are fixed. }
% 	\label{fig:Interpolant_DNNrepresentation}
% \end{figure}

% \textbf{HiDeNN}

% For HiDeNN, all shape functions are represented by DNNs and then assembled together. Nodal values are introduced as weights in the last layer. Weights and biases in the shape function part, i.e., part surrounded by dashed line in Fig. \ref{fig:Interpolant_DNNrepresentation}(a), are constraint and depend on nodal positions $x_I^*$. Nodal values are free except boundary conditions. In the optimization, weights and biases are obtained by optimizing nodal positions $x_I^*$ and nodal values, i.e.,
% \begin{eqnarray}\label{eq:PE_minimization}
%     \text{find} && \mathscr{u}_I, \bm{x}_I^*\\ \nonumber
%     \text{min} && Loss(u^h) \\ \nonumber 
%     \text{where} && \mathscr{u}^{h}= \sum^{np}_{I=1}\mathscr{N}_I(\bm{x}^{*}_{I},x,\mathscr{A})\mathscr{u}_{I} \\ \nonumber
%     \text{and} && \sum^{np}_{I=1}\mathscr{N}_I(\bm{x}^{*}_{I},x,\mathscr{A}) = 1.
% \end{eqnarray}

% \textbf{FEM}

% Following the way in HiDeNN, shape functions can be rewritten in a DNN format. The difference is that weights and biases in this part, i.e., surrounded by red solid line in Fig. \ref{fig:Interpolant_DNNrepresentation}(b), are fixed and determined by given mesh. The optimization variable is merely nodal value in the last layer. The optimization formula is
% \begin{eqnarray}\label{eq:PE_minimization}
%     \text{find} && \mathscr{u}_I,\\ \nonumber
%     \text{min} && Loss(u^h) \\ \nonumber 
%     \text{where} && \mathscr{u}^{h}= \sum^{np}_{I=1}\mathscr{N}_I(x)\mathscr{u}_{I} \\ \nonumber
%     \text{and} && \sum^{np}_{I=1}\mathscr{N}_I(x) = 1.
% \end{eqnarray}

% \textbf{Neural network based methods}

% We use the same structure for NN-based methods for comparison as illustrated in Fig. \ref{fig:Interpolant_DNNrepresentation}(c). Here all weight and biases are free to be optimized, and there are no concepts of shape functions and nodal values. The optimization is straightforward to be
% \begin{eqnarray}\label{eq:PE_minimization}
%     \text{find} && \bm{W},\bm{b}\\ \nonumber
%     \text{min} && Loss(u^h) \\ \nonumber 
%     \text{where} && \mathscr{u}^{h}= u^h(\bm{W},\bm{b},x,\mathscr{A}).
% \end{eqnarray}

% \textbf{Modal superposition}

% According to (\ref{eq:MSExpand}), multidimensional shape functions of MS are the product of 1D shape functions, which are also fixed and determined by nodal positions along each direction. Nodal values are constraint in the form of tensor product, i.e.,
% \begin{equation}
%     u_{i,j,k}=\sum_{q=1}^{Q}\beta^{(q)}_{i}\gamma^{(q)}_j\theta^{(q)}_k.
% \end{equation}
% The optimization is
% \begin{eqnarray}
%     \text{find} && \beta^{(q)}_i, \gamma^{(q)}_j, \theta^{(q)}_k,\\ \nonumber
%     \text{min} && Loss(u^h) \\ \nonumber 
%     \text{where} && \mathscr{u}^{h}= \sum_{i=1}^{n_1}\sum_{j=1}^{n_2}\sum_{k=1}^{n_3} \mathscr{N}_i(x) \mathscr{N}_j(y) \mathscr{N}_k(z) \left( \sum_{q=1}^Q \beta^{(q)}_i \gamma^{(q)}_j \theta^{(q)}_k \right) \\ \nonumber
%     \text{and} && \sum^{n_1}_{i=1}\mathscr{N}_i(x) = 1, \sum^{n_2}_{j=1}\mathscr{N}_j(y) = 1, \sum^{n_3}_{k=1}\mathscr{N}_k(z) = 1.
% \end{eqnarray}



\section{Error analysis of FEM, CD, HiDeNN and NN-based solutions for PDEs}

We consider a partial differential equation with homogeneous boundary conditions
\begin{equation}
\left\{\begin{array}{l}
    \mathcal{L}\bm{u}(\bm{x})+\bm{b}(\bm{x})=0 \text{ in } \Omega \subset \mathbb{R}^d, \\
    \bm{u}|_{\partial \Omega}=\bm{0},
\end{array}\right.
\label{eq:GeneralPDE}
\end{equation}
where $\bm{u}\in \mathbb{R}^m$ denotes an $m$-dimensional vector-valued function in a certain Hilbert space $H(\mathbb{R}^d, \mathbb{R}^d)$, $\bm{b}$ the source term, $\bm{x} \in \mathbb{R}^d$ the $d$-dimensional space coordinates, and $\mathcal{L}$ a second-order differential operator.

We assume that an energy potential $\Pi(u)$ exists, formulated in the following form
\begin{equation}
    \Pi(\bm{u})=\dfrac{1}{2}a(\bm{u},\bm{u})-(\bm{b},\bm{u}),
\end{equation}
where $a(\cdot , \cdot)$ is the symmetric and bilinear form corresponding to the second-order differential operator $\mathcal{L}$, and $(\bm{f},\bm{g})=\int_{\Omega} \bm{f} \cdot \bm{g} \mathrm{d}\bm{x}$ denotes the inner product. For example, let $a(\bm{f},\bm{g})=\int_{\Omega} \nabla \bm{f} \cdot \nabla \bm{g} \mathrm{d}\bm{x}$ for Poisson equation, 
The minimization of $\Pi(u)$ gives the solution to \eqref{eq:GeneralPDE}. This leads to a weak form of  \eqref{eq:GeneralPDE}, which reads
\begin{equation}
    \bm{u}=\argmin_{\bm{u}^* \in H(\mathbb{R}^m, \mathbb{R}^n)} \Pi[\bm{u^*}]
\end{equation}


Such a weak form is commonly adopted in interpolation theory based numerical approaches, such as the methods shown in Section 2. Denoted by $\mathcal{S}^h \subset H(\mathbb{R}^d, \mathbb{R}^m)$ the discretized approximation solution set with a characteristic mesh size $h$, the approximate solution based a given interpolation function set is then
\begin{equation}
    \bm{u}^h=\argmin_{\bm{u}^{h*} \in \mathcal{S}^h} \Pi[\bm{u^{h*} }]
\end{equation}
In the following, we shall take $\mathcal{S}^h$ to be $\mathcal{M}_{0,Q}^h, \mathcal{V}_0^h, \mathcal{H}_0^h, \mathcal{N}_0^h$ , which are the subsets of $\mathcal{M}_Q^h, \mathcal{V}^h, \mathcal{H}^h, \mathcal{N}^h$ under homogeneous boundary conditions,  respectively. 

\subsection{Error analysis}

We assert the following relations among error bounds for FEM, NN, HiDeNN and CD
\begin{equation}
    \left\| u^{CD}-u^{exact} \right\|_{E} \geq \left\| u^{FEM}-u^{exact} \right\|_{E} \geq \left\| u^{HiDeNN}-u^{exact} \right\|_{E} \geq \left\| u^{NN}-u^{exact} \right\|_{E},
    \label{eq:ErrorAnalysis}
\end{equation}
Here, $\left\| \cdot \right\|_{E}=\sqrt{a(\cdot,\cdot)}$ is called as the energy norm, and $u^{exact}$ is the real solution of the problem, i.e.,
\begin{equation}
    u^{exact}=\arg \min_{u\in H^1_0} \Pi[u].
\end{equation}

The relationship (\ref{eq:RelationshipAmongMethods}) is inherited by $\mathcal{M}_{0,Q}^h, \mathcal{V}_0^h, \mathcal{H}_0^h, \mathcal{N}_0^h$, i.e.,
\begin{equation}
    \mathcal{M}_{0,Q}^h \subset \mathcal{V}_0^h \subset \mathcal{H}_0^h \subset \mathcal{N}_0^h.
    \label{eq:RelationshipAmongMethodsBC}
\end{equation}

These four methods are all based on the minimal energy principle,
\begin{equation}
    \bm{u}=\arg \min_{\bm{u}^h \in \mathcal{S}^h} \Pi[\bm{u}^h],
\end{equation}
where $\mathcal{S}^h$ is selected as $\mathcal{M}_{0,Q}^h, \mathcal{V}_0^h, \mathcal{H}_0^h, \mathcal{N}_0^h$ for CD, FEM, HiDeNN, and NN, respectively. Thus due to the relationship (\ref{eq:RelationshipAmongMethodsBC}) among them, we have
\begin{equation}
    \Pi[u^{CD}] \geq \Pi[u^{FEM}] \geq \Pi[u^{HiDeNN}] \geq \Pi[u^{NN}].
\end{equation}
This leads to the error bounds (\ref{eq:ErrorAnalysis}). %It indicates yet does not guarantee the accuracy comparison for these methods. As a remedy, we shall compare PGD, FEM, and HiDeNN in the numerical examples.
 We remark that the above theoretical analysis does not account for numerical implementations. For instance, it is not easy to find the minimal value of $\Pi[u^{NN}]$ for NN, although its theoretical results seem better.

==> Part2_Oldversion.tex <==
\section{HiDeNN-PGD}
\label{sec:HiDeNNPGD}

From Section 3, HiDeNN gets better accuracy compared with classical FEM due to the adaptivity of nodal positions. More DoFs might result in more cost. On the other hand, representation of separated variables provide a reduced order model to improve the efficiency but might lose accuracy. Here, we combine HiDeNN and PGD, which might seek for a good balance between accuracy and computational cost. In subsection 5.1, we review HiDeNN formulation. Considering only 1D representation needed in the separated form, we focus on 1D HiDeNN here. And then combine HiDeNN and PGD for multidimensional problem in subsection 5.2. We present the 2D Poisson problem to illustrate the solution scheme.

\subsection{HiDeNN Formulation}
In standard 1D FEM, the computational domain $\Omega$ is descretized by a grid with $n$ nodes and the shape function associated with an internal node $x_I$ is
\begin{equation}
N_I(x)=\left\{
\begin{array}{cc}
\dfrac{x-x_{I-1}}{x_I-x_{I-1}},     & x_{I-1}\leq x \leq x_I, \\
\dfrac{x_{I+1}-x}{x_{I+1}-x_{I}},     & x_I \leq x \leq x_{I+1}, \\
0,   & else where,
\end{array}
\right.
\label{eq:linearshapefunction}
\end{equation}
where $x_{I-1}$ and $x_{I+1}$ are the two neighbor points of the node $\:x_{I}$ from the left side and right side, respectively.

We rewrite $N_I(x)$ in a DNN format consists of weights, biases, and activation functions. Considering the shape function is a piecewise linear function, the activation function is selected as ReLU function, i.e., $\mathscr{A}_{1}=\max(0,x)$. Fig. \ref{fig:1D_DNN_representation}(a) shows the DNN representation of the linear shape function. The corresponding formula is 
\begin{eqnarray}
\mathscr{N}_{I}(x;\bm{W}, \bm{b},\:\bm{\mathscr{A}})
&=& W_{11}^{l=4}\mathscr{A}_{1}\left( W_{11}^{l=3} \mathscr{A}_{1} \left( W_{11}^{l=2}x+b_{1}^{l=2} \right) +b_{1}^{l=3} \right) \\ \nonumber
&&+ W_{21}^{l=4}\mathscr{A}_{1} \left( W_{22}^{l=3} \mathscr{A}_{1} \left( W_{12}^{l=2}x+b_{2}^{l=2} \right) +b_{2}^{l=3} \right) +b_{1}^{l=4}\\ \nonumber
&=& \mathscr{A}_{1}\left( \dfrac{-1}{x_I-x_{I-1}} \mathscr{A}_{1} \left( -x+x_I \right) +1 \right) + \mathscr{A}_{1} \left( \dfrac{-1}{x_{I+1}-x_I} \mathscr{A}_{1} \left( x-x_I \right) +1 \right) -1, \nonumber
\end{eqnarray}
where $\bm{W}=[W_{11}^{l=2},W_{12}^{l=2},W_{11}^{l=3},W_{22}^{l=3},W_{11}^{l=4},W_{21}^{l=4}]$, and $\bm{b}=[b_{1}^{l=2},b_{2}^{l=2},b_{1}^{l=3},b_{2}^{l=3},b_{1}^{l=4}]$ are the weights and biases of the connected neurons. Note that all the weights and biases are functions of nodal coordinates. The formula can be rewritten as the form of
\begin{equation}
    \mathcal{N}_I(\bm{x};\bm{x}_I^*,\bm{\mathscr{A}}),
\end{equation}
where $\bm{x}_I^*$ denotes the vector that represents the neighbor nodes of node $\bm{x}_I$ involved in $N_I(\bm{x})$. For 1D linear shape function, it should be $\bm{x}_I^*=[x_{I-1},\:x_{I},\:x_{I+1}]$. For the sake of clarity, one more layer is added to introduce the nodal value $u_I$, i.e., the formula becomes
\begin{eqnarray}
\mathscr{u}_I^{h}&=&\mathscr{N}_{I} (x;\:\bm{W},\bm{b},\:\bm{\mathscr{A}})\mathscr{u}_{I}=\mathscr{N}_{I} (x;\:\bm{x}_I^*,\:\bm{\mathscr{A}})\mathscr{u}_{I}; \mbox{ no summation on } {I}\\ \nonumber
&=& \mathscr{A}_{0}\left(\mathscr{A}_{1}\left( \dfrac{-1}{x_I-x_{I-1}} \mathscr{A}_{1} \left( -x+x_I \right) +1 \right) -0.5\right) \mathscr{u}_{I} \\ \nonumber
&&+ \mathscr{A}_{0}\left(\mathscr{A}_{1} \left( \dfrac{-1}{x_{I+1}-x_I} \mathscr{A}_{1} \left( x-x_I \right) +1 \right) -0.5\right) \mathscr{u}_{I},
\end{eqnarray}
where $\mathscr{u}_I^{h}$ and $\mathscr{u}_I$ are the interpolated displacement and nodal displacement at node $x_I$, $\bm{\mathscr{A}}=[\mathscr{A}_{0},\:\mathscr{A}_{1}]$ are the activation functions used for the construction of the DNN approximation. $\mathscr{A}_{0}(x)=x$ is an identical function. Fig. \ref{fig:1D_DNN_representation}(b) gives the DNN representation of the interpolation of the nodal displacement at node $x_I$.

\begin{figure}[h]
	\centering
	\subfigure[DNN-based 1D shape function]{\includegraphics[width=0.42\textwidth]{global_shape_func_DNN.png}}
	\hspace{0.1in}
	\subfigure[DNN-based 1D interpolation function ]{\includegraphics[width=0.5\textwidth]{interpolation_func_DNN.png}}
	\caption{Deep neural network (DNN) representation of the 1D global shape function and interpolation function.}
	\label{fig:1D_DNN_representation}
\end{figure}

Once the shape function with nodal value for an arbitrary node $x_I$ is constructed, the interpolation is obtained by assembling all DNNs together, i.e.,
\begin{equation}
\mathscr{u}^{h}(x)=\sum_{I=1}^{n}\mathscr{N}_{I} (x;\:\bm{x}_I^*,\:\bm{\mathscr{A}})\mathscr{u}_{I}.
\end{equation}
Compared with classical FEM, nodal positions are introduced as additional DoFs in the optimization for HiDeNN, which increases both the local and global accuracy of the interpolants.

Reference \cite{zhang2020hierarchical} also presented the DNN representation of various rational functions including Lagrange polynomials, B-spline, Reproducing Kernel Particle Method (RKPM), NURBS, Isogeometric analysis (IGA), etc., and multidimensional shape functions.

\subsection{Reduced order HiDeNN via PGD}

HiDeNN obtains better results than classical FEM with fixed number of nodes because of adaptive mesh. \COMMENT{Now we can also relax nodal positions in each dimension in the PGD for regular mesh.} The shape functions in each direction are written in the DNN format, namely, (\ref{eq:MSDisX}-\ref{eq:MSDisZ}) are replaced by 1D HiDeNN interpolants,
\begin{eqnarray}
    X^{(q)}(x)&=&\sum_{I=1}^{n_1} N_I(x;\bm{x}_I^*,\bm{\mathcal{A}})\beta_I^{(q)}, \\
    Y^{(q)}(y)&=&\sum_{J=1}^{n_2} N_J(y;\bm{y}_J^*,\bm{\mathcal{A}})\gamma_J^{(q)}, \\
    Z^{(q)}(z)&=&\sum_{K=1}^{n_3} N_K(z;\bm{z}_K^*,\bm{\mathcal{A}})\theta_K^{(q)}.
\end{eqnarray}
Thus the interpolation function set is defined by
\begin{eqnarray}
    \mathcal{G}_Q^h=&\Bigg \{ &u^h \bigg |u^h=\sum_{q=1}^Q \left( \sum_{I=1}^{n_1} N_I(x;\bm{x}_I^*,\bm{\mathcal{A}})\beta_I^{(q)} \right) \left( \sum_{J=1}^{n_2} N_J(y;\bm{y}_J^*,\bm{\mathcal{A}})\gamma_J^{(q)} \right) \left( \sum_{K=1}^{n_3} N_K(z;\bm{z}_K^*,\bm{\mathcal{A}})\theta_K^{(q)} \right) \Bigg \}.
\end{eqnarray}
Since adaptivity occurs only in each direction, the mesh is always regular.

\subsection{Multi-modes solution scheme: the 2D Poisson problem as illustration}

For the sake of simplicity and without loss of generality, we consider 2D Poisson problem,
\begin{equation}
\left\{\begin{array}{l}
    \nabla^2 \bm{u}(x,y)+b(x,y)=0 \text{ in } \Omega_{(x,y)} \subset \mathbb{R}^2, \\
    \bm{u}|_{\partial \Omega}=\bm{0},
\end{array}\right.
\label{eq:PoissonEqHP}
\end{equation}
(\ref{eq:PoissonEqHP}) is solved in the regular domain $\Omega_{(x,y)}=[a,b]\times[c,d]$ with homogeneous boundary conditions. Note that if considering boundary conditions, we can separate the solution into two parts,
\begin{equation}
    u=u^0+\Delta u,
\end{equation}
Where $u^0$ is an arbitrary function satisfying boundary conditions and $\Delta u$ is the solution to the new equations with homogeneous boundary conditions.
The variational formula of (\ref{eq:PoissonEqHP}) is 
\begin{equation}
    \Pi(u)=\dfrac{1}{2}\int_{\Omega_{(x,y)}} (\nabla u)^2 \mathrm{d}x\mathrm{d}y - \int_{\Omega_{(x,y)}} u(x,y)b(x,y) \mathrm{d}x\mathrm{d}y
    \label{eq:PoissonVar}
\end{equation}

Substituting HiDeNN-PGD interpolation function into (\ref{eq:PoissonVar}), we obtain
\begin{eqnarray}
    \label{VariationalHP}
    \Pi(u^h)&=&\dfrac{1}{2}\sum_{p=1}^Q\sum_{q=1}^Q \left(\int_{x_1}^{x_{n_1}} \dfrac{d}{dx}X^{(p)}(x)\dfrac{d}{dx}X^{(q)}(x) \mathrm{d}x\right) \left(\int_{y_1}^{y_{n_2}} Y^{(p)}(y)Y^{(q)}(y) \mathrm{d}y\right) \\ \nonumber
    &+&\dfrac{1}{2}\sum_{p=1}^Q\sum_{q=1}^Q \left(\int_{x_1}^{x_{n_1}} X^{(p)}(x)X^{(q)}(x) \mathrm{d}x\right) \left(\int_{y_1}^{y_{n_2}} \dfrac{d}{dy}Y^{(p)}(y) \dfrac{d}{dy}Y^{(q)}(y) \mathrm{d}y\right) \\ \nonumber
    &-&\sum_{q=1}^Q\int_{\Omega_{(x,y)}} X^{(q)}(x)Y^{(q)}(y) b(x,y)\mathrm{d}x\mathrm{d}y,
\end{eqnarray}
with the discrete mesh $[x_1=a, x_2, \cdots, x_{n_1}=b]\times[y_1=c,y_2,\cdots,y_{n_2}=d]$.
Notice that there exist cross terms in Eq.(\ref{VariationalHP}). For convenience and considering the difficulties to do exact integration between different discrete meshes, all the modes share the same mesh $[x_1,x_2,\cdots,x_{n_1}]\times[y_1,y_2,\cdots,y_{n_2}]$ and the same shape functions. We use Gaussian numerical integration for the source term.

Once the interpolation function is obtained, minimal variational principle gives the approximated solution. The process in HiDeNN-PGD is formulated as
\begin{eqnarray}
    \text{find} && \beta_I^{(1)}, \gamma_J^{(1)},\cdots,\beta_I^{(Q)}, \gamma_J^{(Q)}, x_I, y_J,I=1,\cdots,n_1, J=1,\cdots,n_2\\ \nonumber
    \text{min} && \dfrac{1}{2}\int_{\Omega_{(x,y)}} (\nabla u)^2 \mathrm{d}x\mathrm{d}y - \int_{\Omega_{(x,y)}} u(x,y)b(x,y) \mathrm{d}x\mathrm{d}y \\ \nonumber
    && u^h=\sum_{q=1}^Q \left( \sum_{I=1}^{n_1} N_I(x;\bm{x}_I^*,\bm{\mathcal{A}})\beta_I^{(q)} \right) \left( \sum_{J=1}^{n_2} N_J(y;\bm{y}_J^*,\bm{\mathcal{A}})\gamma_J^{(q)} \right) \\ \nonumber
    \text{and} && \sum^{n_1}_{I=1}\mathscr{N}(\bm{x}^{*}_{I},x,\mathscr{A}) = 1, \sum^{n_2}_{J=1}\mathscr{N}(\bm{y}^{*}_{J},y,\mathscr{A}) = 1.
\end{eqnarray}
The gradient descent method is applied to iteratively minimize $\Pi(\mathscr{u}^h)$ and solve for all parameters together. In the following numerical examples, we choose the Adam algorithm \cite{kingma2014adam}, i.e.,
\begin{framed}
	\begin{enumerate}
		\item Initialization: Set number of modes $Q$, initial nodal positions $x_I,y_J,I=1,2,\cdots,n_1,J=1,2,\cdots,n_2$, initial coefficients $\beta^{(q)}_I,\gamma^{(q)}_J, q=1,2,\cdots,Q$ and maximal iteration step $M$
		\item Algorithm: 
		
		While $k\leq M$ do
		\begin{enumerate}
		    \item Compute gradient $\dfrac{\partial}{\partial x_I}, \dfrac{\partial}{\partial y_J}, \dfrac{\partial}{\partial \beta_I^{(q)}},
		    \dfrac{\partial}{\partial \gamma_J^{(q)}}, I=1,\cdots,n_1, J=1,\cdots,n_2, q=1,\cdots,Q$;
		    \item Update $x_I,y_J,\beta_I^{(q)},\gamma_J^{(q)},I=1,\cdots,n_1, J=1,\cdots,n_2, q=1,\cdots,Q$ by using Adam algorithm;
		\end{enumerate}
		End while.
	\end{enumerate}
\end{framed}


\subsection{Error bounds for HiDeNN-PGD}

% \begin{figure}[h]
% 	\centering
% 	\includegraphics[width=0.8\textwidth]{RelationshipFiveMethods.png}
% 	\caption{Illustration for updated relationship among interpolation function sets of MS, FEM, HiDeNN-PGD, HiDeNN and NN. When $Q$ is big enough, FEM interpolation set $\mathcal{V}^h$ is the subset of HiDeNN-PGD one $\mathcal{G}^h_Q$.}
% 	\label{fig:RelationshipHiDeNNPGD}
% \end{figure}
We proposed HiDeNN-PGD in this section. Then we can put it in our comparion among several methods. The relationship of several interpolation function sets is illustrated in Fig. \ref{fig:Relationship}. HiDeNN-PGD requires the mesh regular, while HiDeNN optimizes nodal positions freely, so $\mathcal{G}^h_Q \subset \mathcal{H}^h, \forall Q \in \mathbb{N}$. On the other hand, HiDeNN-PGD has more DoFs than CD under the same number of modes, so $\mathcal{M}^h_Q \subset \mathcal{G}^h_Q, \forall Q \in \mathbb{N}$. Referring to Section 3, when $Q$ is big enough ($Q\geq\min\{n_1,n_2\}$ for 2D and $Q\geq\min\{n_1 n_2,n_2 n_3, n_3 n_1\}$ for 3D), we have $\mathcal{M}^h_Q=\mathcal{V}^h$. Thus,
\begin{equation}
    \mathcal{M}^h_Q=\mathcal{V}^h\subset\mathcal{G}^h_Q \subset \mathcal{H}^h \subset \mathcal{N}^h, 
\end{equation}
with $Q\geq\min\{n_1,n_2\}$ for 2D or $ Q\geq\min\{n_1 n_2,n_2 n_3, n_3 n_1\}$ for 3D.
It leads to 
\begin{eqnarray}
    &&\left\| u^{CD}-u^{exact} \right\|_{E} \geq \left\| u^{FEM}-u^{exact} \right\|_{E} \geq \left\| u^{HiDeNN-PGD}-u^{exact} \right\|_{E} \\ \nonumber
    &&\geq \left\| u^{HiDeNN}-u^{exact} \right\|_{E} \geq \left\| u^{NN}-u^{exact} \right\|_{E},
    \label{eq:ErrorAnalysisUpdate}
\end{eqnarray}
This shows HiDeNN-PGD might reach better accuracy than FEM with regular mesh at increasing number of modes. When $Q$ is small, $\mathcal{M}^h_Q$ is the subset of the intersection of $\mathcal{G}^h_Q$ and $\mathcal{V}^h$.
